Learning Maritime Obstacle Detection from Weak Annotations by Scaffolding

Coastal water autonomous boats rely on robust perception methods for obstacle detection and timely collision avoidance. The current state-of-the-art is based on deep segmentation networks trained on large datasets. Per-pixel ground truth labeling of such datasets, however, is labor-intensive and expensive. We observe that far less information is required for practical obstacle avoidance - the location of water edge on static obstacles like shore and approximate location and bounds of dynamic obstacles in the water is sufficient to plan a reaction. We propose a new scaffolding learning regime (SLR) that allows training obstacle detection segmentation networks only from such weak annotations, thus significantly reducing the cost of ground-truth labeling. Experiments show that maritime obstacle segmentation networks trained using SLR substantially outperform the same networks trained with dense ground truth labels. Thus accuracy is not sacrificed for labelling simplicity but is in fact improved, which is a remarkable result.

==> trash/cutout.tex <==
RESULTS SECTION
------------------------------------------------------------------------------------------
\section{Results}\label{sec:experiments}

\subsection{Experimental setup}\label{sec:experiments/setup}

% MODS:
% - Evaluates water-edge as the boundary between the largest water component and the obstacles.
% - Evaluates obstacle detection

The scaffolding learning regime is evaluated on the most recent maritime obstacle detection benchmark MODS~\cite{Bovcon2020MODS}.
%We perform the evaluation on the recently proposed MODS benchmark~\cite{Bovcon2020MODS}, designed specifically for obstacle detection in the marine domain. 
MODS is based on a diverse and large marine dataset containing approximately 100 annotated sequences captured under varied conditions. The evaluation protocol reflects the detection performance meaningful for practical USV navigation and separately evaluates (i) the accuracy of obstacle-water edge estimation for static obstacles and (ii) the detection performance for dynamic obstacles (in terms of obstacle detection metrics). Water edge estimation is analysed in terms of an localization accuracy (\ie RMSE of the water edge height) and detection robustness (\ie what portion of the water edge is correctly identified), and dynamic obstacle detection is analysed in terms of true positive (TP), false positive (FP) and false negative (FN) detections. The dynamic obstacles count as detected (TP) if the coverage of the segmentation inside the bounding box is sufficient, otherwise the obstacle counts as undetected (FN). Predicted obstacle components outside of dynamic obstacle bounding boxes count as false positive detections. In addition, dynamic obstacle detection is evaluated overall and separately inside the danger zone (\ie within 15m of the USV), where the detection performance is critical for safe USV operation.

In all experiments we train the models on the MaSTr1325 obstacle segmentation dataset~\cite{Bovcon2019Mastr}. For the purposes of this study the MaSTr1325 dataset has been semi-automatically re-annotated following the obstacle-oriented annotation scheme. During training we apply random image augmentation to the input images as in \cite{Bovcon2019Mastr}. The models are trained using the RMSProp optimizer with a momentum of 0.9, initial learning rate $10^{-6}$ and standard polynomial reduction decay of 0.9. The total batch size is 12. 

To analyse parts of our training approach we use our obstacle-oriented training regime to train a WaSR segmentation model~\cite{Bovcon2020WaSR}, designed specifically for obstacle detection in the marine domain. We denote this model WaSR$_W$. ResNet-101 is used as the encoder of the WaSR model. Features $\mathbf{F}$ are extracted from the output of the third (next-to-last) residual convolutional block of the encoder. For both the warm-up and re-training steps, the encoder is pretrained on the COCO dataset (\ie weights of a pretrained DeepLab encoder are used) and the decoder is initialized randomly. Focal loss $L_\mathrm{foc}$ with the focusing parameter $\gamma = 2$ is used. We set the hyperparameters $\lambda_1 = \lambda_2 = 1$, $\beta_W = 0.125$, $\theta_W = 45$ and $\beta_S = 20$. In a preliminary study we determined that the performance of the model is not sensitive to exact values of the hyperparameters.
The model warm-up is executed for 25 epochs and the re-training is run for 50 epochs.

\subsection{Ablation study}\label{sec:experiments/ablation}

\begin{table*}
\caption{Ablation study of the components of the proposed obstacle-oriented model supervision. Removing: constraint consolidation ($\bar{\mathrm{C}}$), aspects of model introspection ($\mathrm{I}_P$, $\bar{\mathrm{I}}$ and $\bar{\mathrm{I}}+$) and the pairwise loss term ($\overline{\mathrm{PA}}$). Performance is measured in terms of water-edge estimation accuracy ($\mu_\mathrm{A}$), robustness ($\mu_\mathrm{R}$) and obstacle detection precission (Pr), recall (Re) and F1 score. Obstacle detection metrics are measured overall and inside the danger zone.}
\label{table:ablation}
\centering
\begin{tabular}{lccccccccc}
\toprule
 & & \phantom{a} & \multicolumn{3}{c}{Overall} & \phantom{a} & \multicolumn{3}{c}{Danger zone (\textless 15m)} \\
 \cmidrule{4-6} \cmidrule{8-10}
 & $\mu_\mathrm{A}$[px]($\mu_\mathrm{R}$) & & F1 & Pr & Re & & F1 & Pr & Re \\
\midrule
WaSR$_W$                  &  11.3 (98.8) &    &  \textbf{93.5} &  \textbf{96.5} &  90.7 &     &  \textbf{86.1} &  \textbf{79.0} &  94.7 \\
\midrule
$\mathrm{P}_{\bar{\mathrm{C}}}$       &  11.6 (98.7) &    &  92.0 &  93.8 &  90.3 &     &  85.1 &  78.5 &  92.9 \\
$\mathrm{P}_{\bar{\mathrm{F}}}$     &  10.2 (99.0) &    &  91.6 &  93.3 &  90.0 &     &  76.4 &  64.7 &  93.2 \\
$\bar{\mathrm{P}}$       &   9.4 (99.1) &    &  91.4 &  89.4 &  93.5 &     &  57.4 &  41.2 &  94.7 \\
$\bar{\mathrm{P}}+$      &   \textbf{8.9 (99.2)} &    &  91.9 &  89.9 &  \textbf{94.1} &     &  46.3 &  30.4 &  \textbf{97.4} \\
$\overline{\mathrm{PA}}$ &  12.3 (98.7) &    &  92.5 &  93.2 &  91.8 &     &  85.0 &  77.3 &  94.4 \\
\bottomrule
\end{tabular}
\end{table*}

We perform an ablation study to determine the contributions of different components of the learning process. Ablations are performed by disabling individual components at a time (\ie changes do not stack). Results of the study are presented in Table~\ref{table:ablation}. First we analyse two aspects of the dense pseudo label generation process described in Section~\ref{sec:dense_labels}. Specifically, (i) we disable the constraint consolidation steps ($\mathrm{P}_{\bar{\mathrm{C}}}$) and (ii) we skip the feature prototype construction and similairy map computation and use consolidated predictions as the class probabilities directly ($\mathrm{P}_{\bar{\mathrm{F}}}$). Removing the label constraints ($\mathrm{P}_{\bar{\mathrm{C}}}$) slightly reduces the overall performance in all categories (water edge estimation by 2.6\% and obstacle detection by 1.6\%). Performing the model introspection only based on the models predictions ($\mathrm{P}_{\bar{\mathrm{F}}}$) has a much larger impact. This approach leads to a significant drop in performance on obstacle detection (2.05\% overall and 11.9\% inside the danger zone), however it also achieves better water-edge estimation accuracy (+10.2\%) (TODO: mogoče podamo samo rezultate za robustnost?). The obstacle detection performance difference is mainly due to an increased number of FP predictions, which results in a drop in precision.

TODO: razlaga zakaj water edge slabši

Next, we completely disable the pseudo label generation and re-training steps (\ie only warm-up). In addition to a normal warm-up model trained for 25 epochs ($\bar{\mathrm{P}}$), we also train a warm-up model for 75 epochs ($\bar{\mathrm{P}}+$), which is the combined length of the warm-up and re-training phase, to account for the difference in training length. In any case, removing the re-training step results in a massive drop in obstacle detection precision, especially inside the danger zone (-40\% and -60\% for both models respectively), which is a result of high false positive rate (example in Figure~\ref{fig:introspection_comp}) and consequently low precision. This shows that dense pseudo label generation and model re-training is a crucial step in achieving robust obstacle detection. Note also, that the water-edge estimation accuracy of the warm-up models is phenomenal -- it vastly outperform existing state-of-the-art fully-supervised methods, while the re-trained model merely matches their performance in this aspect. This is an interesting finding and further research is needed to investigate, how to retain such water-edge performance during re-training.

\begin{figure}
\centering
\includegraphics[width=\linewidth]{figures/introspection_comp.pdf}
\caption{Effects of the model re-training based on generated pseudo labels. After model warm-up (left), the network tends to predict small false positives (\eg reflections) on unseen data. After the re-training step (right), this behaviour is improved resulting in a much better obstacle detection score.}
\label{fig:introspection_comp}
\end{figure}

Finally, we analyse the contribution of the pairwise loss ($\overline{\mathrm{PA}}$). Disabling the pairwise loss has the smallest effect on obstacle detection performance (-1.1\% F1 overall and -1.3\% inside the danger zone), which is expected, as its purpose is mainly to refine the boundaries between classes and improve segmentation quality, which is not reflected in the obstacle detection metrics. The decrease in segmentation quality is also confirmed by a noticeable drop in water-edge estimation accuracy (8.5\%).



\subsection{Re-training again}

\begin{table}
\caption{Multiple model re-training steps (along with pseudo-label generation) and its effect on model performance. WaSR$_W$, WaSR$_W^{2\times}$ and WaSR$_W^{3\times}$  use 1, 2 and 3 re-training iterations respectively. Performance is measured on the MODS benchmark in terms of water-edge estimation accuracy ($\mu_\mathrm{A}$) and obstacle detection F1 score (overall and inside the danger zone).}
\label{table:num_iterations}
\centering
\begin{tabular}{lcc}
\toprule
 & $\mu_\mathrm{A}$[px] & F1 \\
\midrule
WaSR$_W$        &  \textbf{11.3} &  \textbf{93.5} (86.1) \\
WaSR$_W^{2\times}$    &  11.5 &  93.2 (85.4) \\
WaSR$_W^{3\times}$    &  11.8 &  93.0 (\textbf{86.3}) \\
\bottomrule
\end{tabular}
\end{table}

In this section we investigate if additional pseudo-label-generation and re-training steps lead to additional improvements. We compare models WaSR$_W$, WaSR$_W^{2\times}$ , WaSR$_W^{3\times}$ using 1, 2 or 3 iterations of the model re-training respectively. Pseudo labels for each additional iteration are generated from the features and predictions of the previous model iteration as described in Section~\ref{sec:dense_labels}. Each re-training iteration is trained for 50 epochs. 

Results are presented in Table~\ref{table:num_iterations}. All models achieve comparable performance (variation in the water-edge estimation accuracy is less than 5\% and F1 score variation is less than 1\%). This suggests that benefits of the model re-training saturate after a single  (WaSR$_W$) and no additional benefits are gained by increasing the number of iterations. TODO: povemo, da se zato odločimo za eno iteracijo?

\subsection{Comparison with state-of-the-art}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{figures/comparison.pdf}
\caption{WaSR (fully-supervised) vs. WaSR$_W$ (our) segmentation quality on the MODS benchmark. In the first and second example WaSR produces false positive detections on water reflections of obstacles. WaSR-WS is more robust to such errors. WaSR-WS also works in difficult scenarios including wakes (3) and heavy reflections (4). WaSR-WS produces slightly less accurate obstacle boundary segmentation, especially the sky-obstacle separation, which is not crucial for the downstream task. Best viewed on a screen.}
\label{fig:comparison}
\end{figure*}

\begin{table*}
\caption{Comparison of WaSR$_W$ with state-of-the-art fully-supervised semantic segmentation models on the MODS benchmark in terms of water-edge estimation accuracy ($\mu_\mathrm{A}$), robustness ($\mu_\mathrm{R}$) and obstacle detection precission (Pr), recall (Re) and F1 score. Obstacle detection metrics are measured overall and inside the danger zone. Despite using a significantly simpler annotation scheme, WaSR$_W$ outperforms all other methods in terms of obstacle detection by a considerable margin and matches their performance on water-edge estimation.}
\label{table:sota-comparison}
\centering
\begin{tabular}{lccccccccc}
\toprule
 & & \phantom{a} & \multicolumn{3}{c}{Overall} & \phantom{a} & \multicolumn{3}{c}{Danger zone (\textless 15m)} \\
 \cmidrule{4-6} \cmidrule{8-10}
 & $\mu_\mathrm{A}$[px]($\mu_\mathrm{R}$) & & F1 & Pr & Re & & F1 & Pr & Re \\
\midrule
\multicolumn{10}{@{}l}{\textit{Fully-supervised}} \\
RefineNet                  &  11 (97.3) &    &  91.0 &  89.0 &  \textbf{93.0} &     &  61.8 &  45.1 &  98.1 \\
DeepLabV3~\cite{Chen2018DeepLab}                   &  \textbf{10} (96.8) &    &  86.0 &  80.1 &  92.7 &     &  31.3 &  18.6 &  \textbf{98.4} \\
BiSeNet~\cite{Yu2018Bisenet}                    &  \textbf{10} (97.4) &    &  90.2 &  90.5 &  89.9 &     &  69.1 &  53.7 &  97.0 \\
WaSR~\cite{Bovcon2020WaSR}  &  11 (\textbf{98.9}) &    &  92.6 &  95.5 &  89.9 &     &  75.0 &  62.8 &  92.9 \\
\midrule
\multicolumn{10}{@{}l}{\textit{Obstacle-oriented}} \\
DeepLabV3$_W$ (our) &  12 (98.8) &    &  90.5 &  94.1 &  87.2 &     &  83.3 &  74.1 &  95.0 \\
WaSR$_W$ (our)              &  11 (98.8) &    &  \textbf{93.5} &  \textbf{96.5} &  90.7 &     &  \textbf{86.1} &  \textbf{79.0} &  94.7 \\
\bottomrule
\end{tabular}
\end{table*}

In this section we compare models trained from obstacle annotations using the proposed approach with state-of-the-art models for obstacle segmentation in the marine domain trained in a fully-supervised way. Specifically we compare our methodology against general semantic segmentation models RefineNet, DeepLabV3, BiSeNet and against WaSR, specifically designed for the marine domain. For comparison, we train a DeepLabV3 and a WaSR model (denoted DeepLabV3$_W$ and WaSR$_W$ respectively) using only obstacle annotations, following the same setup as described in Section~\ref{sec:experiments/setup}. ResNet-101 is used as the backbone of DeepLabV3 and features $\mathbf{F}$ are extracted from the third (next-to-last) convolutional residual block as in WaSR$_W$. Fully-supervised models are trained on the fully-annotated MaSTr1325 dataset as described in \cite{Bovcon2020MODS}. Note, that we report the results of our implementation of WaSR, which slightly outperforms the performance reported in \cite{Bovcon2020MODS}.

The results are presented in Table~\ref{table:sota-comparison}. Both models outperform their fully-supervised counter-parts by a considerable margin on obstacle detection and achieve similar performance on the water edge estimation task. Namely, WaSR$_W$ achieves +1.0\% F1 score overall and +14.8\% inside the danger zone compared to WaSR, while DeepLabV3$_W$ achieves +5.1\% F1 score overall and +93.4\% inside the danger zone. The results are somewhat surprising, given that obstacle oriented methods are trained on a drastically simplified annotation scheme consisting only of obstacle bounding boxes and the water-obstacle edge. We find that models trained from obstacle annotations tend to be much more robust and achieve much greater detection precision without significant loss in detection recall. For example in DeepLabV3$_W$ the precision inside the danger zone is increased from 18.6\% (DeepLabV3) to 74.1\% while the recall drops from 98.4\% to 95.0\% resulting in a much better overall performance. This is mainly due to the reduction in the number of false positive detections, to which fully-supervised models seem to be much more sensitive (see Figure~\ref{fig:comparison}). Note also, that fully-supervised models tend to perform slightly better in terms of water-edge estimation. However, as we have demonstrated in Section~\ref{sec:experiments/ablation}, this might not be an inherent weakness of the obstacle-oriented approach.

\subsection{Improving full supervision}

\begin{table}
\caption{Adding weak supervision components to the fully-supervised model. Performance is measured on the MODS benchmark in terms of water-edge estimation accuracy ($\mu_\mathrm{A}$) and obstacle detection F1 score, measured overall and inside the danger zone.}
\label{table:fs-ablation}
\centering
\begin{tabular}{lcc}
\toprule
 & $\mu_\mathrm{A}$[px] & F1 \\
\midrule
WaSR                      &  \textbf{11.0} &  92.6 (75.0) \\
+ pairwise loss           &  11.8 &  88.4 (72.2) \\
+ re-training     &  11.2 &  \textbf{93.1} (\textbf{84.4}) \\
\bottomrule
\end{tabular}
\end{table}

Finally, we investigate if the proposed re-training process can also be applied to full-supervision. Specifically, we compute dense pseudo labels (Section~\ref{sec:dense_labels}) based on the fully-supervised model predictions and features. To disentangle the contribution of the pairwise loss term, we separately train a fully-supervised WaSR model with the sole addition of the pairwise loss. Results are presented in Table~\ref{table:fs-ablation}. 

We find that adding a pairwise loss to a full supervision process negatively affects the performance (-4.6\% F1 score overall). Using a full re-training process, however, we observe similar benefits to the obstacle oriented approach. Namely, improved obstacle detection robustness (F1 +0.5\%), especially inside the danger zone (F1 +9.5\%). This suggests that the re-training through feature annotated pseudo-labels has general regularization properties, even when full segmentation labels are available. Note, however, that the performance still lags behind WaSR$_W$ trained only on obstacle annotation, which indicates that reducing the complexity of the annotations and harnessing that information during model warm-up also offers some additional benefits to full-supervision in terms of obstacle detection.
------------------------------------------------------------------------------------------
